PQS (Prune, Quantize, and Sort): Low-Bitwidth Accumulation of Dot Products in Neural Network Computations

We present PQS, which uses three techniques together - Prune, Quantize, and Sort - to achieve low-bitwidth accumulation of dot products in neural network computations. In conventional quantized (e.g., 8-bit) dot products, partial results are accumulated into wide (e.g., 32-bit) accumulators to avoid overflows when accumulating intermediate partial sums. However, such wide accumulators increase memory bandwidth usage and reduce energy efficiency. We show that iterative N:M pruning in floating point followed by quantization to 8 (or fewer) bits, and accumulation of partial products in a sorted order ("small to large") allows for accurate, compressed models with short dot product lengths that do not require wide accumulators. We design, analyze, and implement the PQS algorithm to eliminate accumulation overflows at inference time for several neural networks. Our method offers a 2.5x reduction in accumulator bitwidth while achieving model accuracy on par with floating-point baselines for multiple image classification tasks.

==> eval.tex <==
\begin{figure*}[ht]
    \subfloat{\label{fig:amd_dram}{\includegraphics[width=0.33\textwidth]{figures/pqs_vs_a2q_mobilenet.pdf}}}\hfill
    \subfloat{\label{fig:amd_perf}{\includegraphics[width=0.31\textwidth]{figures/pqs_vs_a2q_resnet.pdf}}}\hfill
    \subfloat{\label{fig:amd_cache_bw}{\includegraphics[width=0.31\textwidth]{figures/placeholder.pdf}}}\hfill
\caption{
We visualize the trade-off between accumulator bit width and task performance using Pareto frontiers. We observe
that PQS (blue) achieves a lower accummulator bit width bound than A2Q, without sacrificing significant model performance w.r.t to a floating-point baseline
} 
\label{fig:amd}
\vspace{-4mm}
\end{figure*}


==> pq_vs_qp.tex <==
\begin{figure*}[ht]
    \subfloat{\label{fig:amd_dram}{\includegraphics[width=0.33\textwidth]{figures/rosko_vs_qat_new_acc_low_rank.pdf}}}\hfill
    \subfloat{\label{fig:amd_perf}{\includegraphics[width=0.31\textwidth]{figures/pq_qp_mobilenet.pdf}}}\hfill
    \subfloat{\label{fig:amd_cache_bw}{\includegraphics[width=0.31\textwidth]{figures/pq_qp_resnet.pdf}}}\hfill
\caption{
In (a), we compare accuracy of pruning before quantization (P->Q) with quantization before pruning (Q->P) under low-rank approximations of weight matrices in a two-layer MLP.
In comparison to Q->P, P->Q models are more resilient to low-rank weight approximations and suffer from less accuracy loss as sparsity increases.
For larger networks such as MobileNetV2 (b) and ResNet18 (c) on CIFAR10, we see a similar trend when using full-rank weights. 
} 
\label{fig:rank}
\vspace{-4mm}
\end{figure*}

